Control-Aware Transmit Power Allocation for 6G In-Factory Subnetwork Control Systems

In this paper, we develop a novel power control solution for subnetworks-enabled distributed control systems in factory settings. We propose a channel-independent control-aware (CICA) policy based on the logistic model and learn the parameters using Bayesian optimization with a multi-objective tree-structured Parzen estimator. The objective is to minimize the control cost of the plants, measured as a finite horizon linear quadratic regulator cost. The proposed policy can be executed in a fully distributed manner and does not require cumbersome measurement of channel gain information, hence it is scalable for large-scale deployment of subnetworks for distributed control applications. With extensive numerical simulation and considering different densities of subnetworks, we show that the proposed method can achieve competitive stability performance and high availability for large-scale distributed control plants with limited radio resources.

==> RESULTS/runtime.tex <==
\begin{tikzpicture}[scale=0.90]

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{red}{RGB}{255,0,60}
\definecolor{blue}{RGB}{0,0,255}
\definecolor{lightgray204}{RGB}{255,255,255}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.0,0.7)},
  anchor=south west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
ylabel = {Time(ms)},
x grid style={darkgray176},
xmajorgrids,
xmin=42.5, xmax=207.5,
xtick style={color=black},
y grid style={darkgray176},
xlabel = {Number of subnetworks},
ymajorgrids,
ymin=1.34199541807175, ymax=43.8010907769203,
ytick style={color=black}
]
\addplot [dashed, red, mark=o, mark size=3, mark options={solid}]
table {%
50 3.60772442817688
60 4.00972652435303
70 4.32450103759766
80 4.34334278106689
90 4.72414207458496
100 5.00572490692139
110 5.31423425674438
120 5.65466403961182
130 5.91401290893555
140 6.02741861343384
150 6.31173086166382
160 6.58063745498657
170 6.9404935836792
180 7.24755191802979
190 7.54800128936768
200 7.85946798324585
};
\addlegendentry{GGNN}

\addplot [dashed, teal, mark=triangle, mark size=3, mark options={solid}]
table {%
50 3.27195429801941
60 4.36027574539185
70 4.93752956390381
80 5.5459098815918
90 6.5501708984375
100 7.63566970825195
110 8.77511024475098
120 9.74986553192139
130 10.8464908599854
140 11.9308700561523
150 13.2322483062744
160 14.4715852737427
170 16.3326377868652
180 17.7110958099365
190 19.4075908660889
200 21.0409393310547
};\addlegendentry{CGC}

\addplot [dashed, blue, mark=+, mark size=3, mark options={solid}]
table {%
50 9.76164817810059
60 11.6957693099976
70 13.9707870483398
80 15.6113710403442
90 17.4726963043213
100 19.5271015167236
110 21.3734550476074
120 23.5450477600098
130 25.7252159118652
140 27.6036434173584
150 29.5222969055176
160 31.8150978088379
170 34.9156913757324
180 37.2278022766113
190 40.1598892211914
200 41.8711318969727
};\addlegendentry{SISA}

\end{axis}

\end{tikzpicture}
